Robust Head-Pose Estimation Based on Partially-Latent Mixture of Linear Regressions

Head-pose estimation has many applications, such as social event analysis, human-robot and human-computer interaction, driving assistance, and so forth. Head-pose estimation is challenging because it must cope with changing illumination conditions, variabilities in face orientation and in appearance, partial occlusions of facial landmarks, as well as bounding-box-to-face alignment errors. We propose tu use a mixture of linear regressions with partially-latent output. This regression method learns to map high-dimensional feature vectors (extracted from bounding boxes of faces) onto the joint space of head-pose angles and bounding-box shifts, such that they are robustly predicted in the presence of unobservable phenomena. We describe in detail the mapping method that combines the merits of unsupervised manifold learning techniques and of mixtures of regressions. We validate our method with three publicly available datasets and we thoroughly benchmark four variants of the proposed algorithm with several state-of-the-art head-pose estimation methods.

==> AnswerReviewer2.tex <==
\pagestyle{empty}
\onecolumn

\begin{coverletter}{Robust Head Pose Estimation Based on Partially-Latent Mixture of Linear Regressions}{TIP-15272-2016}

\begin{answereditor}{Based on the enclosed set of reviews, I am recommending that the manuscript undergo a second round of MAJOR REVISIONS (RQ). As you will see, while the comments are mostly supportive, one of the reviewers continues to have serious issues, in particular in regards with the overlap between the content of the current submission and your publication cited as [10] therein. I would appreciate if within your next response letter you would pay particular attention to this aspect in order to help me reach a final decision.}

The comments of the three reviewers were positively considered and very seriously taken into account. The paper was edited by a native English speaker/scientist who confirmed our use of hyphenated words. We carefully addressed the concerns and comments of the reviewers concerning the technical content of the paper. We revised the paper to comply with their comments. Here is a summary of our responses and the list of changes:
\begin{itemize}
\item
It is absolutely true that the methodology used in this submission uses the results of [10]. We clearly state this in the submission : page 2 starting at line 57 and continued on the second column. We made an effort to summarize [10] such that the submission is self-consistent. We describe the method such that it can be easily understood by image processing researchers and practitioners, we removed some statistical theoretic aspects, and we summarized the algorithmic aspects of the method. Please see our detailed answer to Reviewer 3 (question~2). In an effort to better justify the use of an inverse Gaussian mixture of linear regressions with partially-latent output, we added one paragraph \refcm{inverse-def} and revised an existing paragraph \refcm{label-prob-1}.

\item
The concept of latent variable associated with regression output seems to be misunderstood by two reviewers. A latent variable has a mathematical/statistical meaning but it does not necessarily have a physical meaning, such as a physical parameter. For example, methods such as principal component analysis (PCA) and the like, map a high-dimensional space onto a latent low-dimensional subspace, but the latter does not necessarily have a physical meaning. For example, if one applies PCA to the high-dimensional HOG features, a low-dimensional representation is obtained but this representation does not correspond to the desired output, e.g. head pose.

The originality of our contribution is to \textbf{train} the regression when the output variable is a concatenation of an observed part and of a latent part. Please see our detailed answers to Reviewer 3 (question~1) and Reviewer 4 (question 1) as well as the revised paragraph \refcm{label-prob-1}

\item
Reviewer 3 complains about section III.C (Forward Predictive Distribution), which has been shortened considerably, page 5. The reviewer states: \textit{``I still think that it makes no sense of Section III.C as there is no experiments about this subsection.''} \textbf{This is absolutely not correct.}  All the experiments are based on cross-validation. The datasets are split into two parts: one part for training and one part for testing (prediction). Section III.C provides the prediction (test) formulae for all the experiments in the paper. In order to clarify this point, we added a paragraph and a description of the algorithm that uses the equations of Section III.C, namely \textbf{Algorithm~\ref{Alg:iterative}} and the associated text \refcm{label-impl-1}. 

\item
Reviewer 4 has a number of questions concerning the use of high-to-low regression, the number of model parameters, and how the number of affine transformations, $K$, is selected. In addition to the experimental validation using the MAE (mean absolute error) we now use the BIC score to find an optimal value for $K$. We added a figure and a new paragraph that explains this and discusses the complexity of the model with respect to $K$, as well as the problem of overfitting when $K$ (and hence the number of parameters) is too large, namely \textbf{Figure~\ref{fig:bic}} and paragraph \refcm{label-exp-1}. Please see our detailed answer to Reviewer 4 (question~2).

\end{itemize}

\end{answereditor}

\begin{answerreviewer2}{1}{AQ - Publish In Minor, Required Changes}
	\qa{I am disappointed with the authors' response, in particular as regards the quality of their English.  The authors' "analysis" demonstrates a profound lack of grasp of English which results in a complete mess when they try to infer regularities from examples.  To explain this in detail is not within the scope of what I see as my duty as a reviewer.  I would only highly advise the authors to implement the linguistic changes I suggested as, as I noted, their understanding of the grammar and the structure of English is clearly not good.  At the same time I do not feel that it would be appropriate for me to reject the paper on this basis and trust that the issues I raised will be dealt with by the production staff.  As I noted in my original review I am happy with the technical contents, so I am reasonably happy to recommend acceptance.  I suggest minor review to allow the authors another chance to modify the paper.}
	{The paper was edited by a native English speaker/scientist. We tried as much as we could to adhere to the hyphenation rules described in the Oxford dictionary \url{https://en.oxforddictionaries.com/punctuation/hyphen}. In particular, one can read on their website: \textit{It's important to use hyphens in compound adjectives describing ages and lengths of time: leaving them out can make the meaning ambiguous. For example, 250-year-old trees clearly refers to trees that are 250 years old, while 250 year old trees could equally refer to 250 trees that are all one year old.}}
\end{answerreviewer2}

\begin{answerreviewer2}{3}{R - Reject}
	\qa{It's just a summary of the paper. For my understanding, I only separate ``the pose parameters'' and
``bounding box shift and phenomena'' as two kind of variables.}
{The pose and bounding box parameters are treated as a multivariate \textbf{observed} random variable, on one side, and \textbf{unobservable phenomena} are treated as a multivariate \textbf{latent} variable, on the other side. The observed variable is denoted with $\Tvect$ and the latent variable is denoted with $\Wvect$. Jointly, they form the \textbf{output} random variable denoted with $\Xvect$. This variable ($\Xvect$) is then modeled with a mixture of Gaussian distributions parameterized by $K$ means, $K$ covariances and $K$ priors.}
	
	\qa{I cannot accept your answer as this paper is just an application of inverse regression [10]. All the formulation
has proposed in [10], the comparison is shown in Line 2 and Line 3 in table 1. Besides, the EM algorithm in
Appendix A is compared to [10] in Line 4-7. The overlapping between this paper and [10] is too much. For a top
journal of IEEE Trans. On Image Processing, it is not acceptable for me.}
{It is absolutely true that the head-pose estimation method proposed in the submitted manuscript uses the statistical method of [10]. This has been clearly stated in the initial submission and in the revised paper. We made an effort to summarize the main algorithmic results of [10]. The similarities of the mathematical formulas pointed out by the reviewer are absolutely normal. By the way, \textbf{some of these formulas correspond to basic probabilistic calculus, they are not original contributions of [10]}. Some statistical theoretic aspects discussed in [10] were removed and we summarized the algorithmic aspects of the method. 

\textbf{Moreover, we thoroughly addressed the pertinence of the use of inverse regression, of high-dimensional to low-dimensional mapping, and of regression with partially latent output in the framework of a computer vision problem.} We described in detail how the method of [10] should be adapted to deal with automatic face detection and not with manually detected faces. This is in itself a major contribution. We also showed that the latent part of the regression output helps to achieve state-of-the-art results. 

It is common practice in an applied field, such as computer vision, to use theoretical results from statistics and applied mathematics.
We note that many state-of-the-art head-pose estimation methods described in the literature make use of existing regression techniques, for example [15] uses random regression forests, [39] uses partial least-squares regression (PLS) [25], [26] uses kernel PLS, [38] uses Gaussian process regression (GPR) [24], and [40] uses support vector regression (SVR) [3]. All these papers describe a well known machine learning method such that the papers are self consistent.

It is unfair to reduce the contribution of our manuscript to the use of inverse regression.

%Similarities were introduce for readers convenience to make the paper self-contained. (We reduce the overlap with [10] and add a paragraph about the iterative estimation of the head pose and bouding box offset to refine the face localization.)\refcm{label-impl-1}
}

	\qa{I still think that it makes no sense of Section III.c as there is no experiments about this subsection. The
formulation compared to [10] is shown in Line 3 in table 1.}
{
Section III.C summarizes the formula of the predictive distribution, which is then used in the paper with the test data. All the experiments described in the paper are composed of two parts: training and testing. \textbf{All the tests reported in the paper (Tables I, II, III) use the forward predictive distribution of Section III.C.}

In an effort to allow the reviewer to better understand the role of the forward predictive distribution, we incorporated the prediction algorithm. Please refer to \textbf{Algorithm~\ref{Alg:iterative}} and the associated text \refcm{label-impl-1}.
%In Section III.a and III.b we are introducing the \textit{low-to-high} regression (\textit{i.e.} from the pose to the observations vectors) and the EM algorithm to learn the parameters of the \textit{low-to-high} regression. But in the end we are interested in estimating the head pose given a new observation, \textit{high-to-low} regression, thus Section III.c is used to explain how we obtain the \textit{high-to-low} regression parameters and also how we achieve a final estimation using them.
}

	\qa{It's good that you make the Z more clear. Although the readers might be familiar with EM or not, it is good to
describe every variable used in the paper. In [10], the Z is described as ``This is modeled by a missing variable Z
such that...'' before Z is used. }
{Indeed, it is important to make a paper self-consistent, even if the concept of a hidden variable is well known in mixture models.}
\end{answerreviewer2}


\begin{answerreviewer2}{4}{AQ - Publish With Minor, Required Changes}
	\qa{Overall,  the method proposed  a  Partially-Latent Mixture of Linear Regressions for head pose estimation. The performance of this method is comparable with the state-of-arts. However, why this method could work well is not well explained, the physical meaning of the latent variable is not clear. I would like to see the physical meaning in the revised version, otherwise, the contribution of this paper is kind of limited even the performance is good.}{The latent part of the output variable has a principled mathematical definition but it does not necessarily have a physical meaning. The main idea of the proposed method relies on the fact that variabilities present in the high-dimensional face descriptor depend on head pose, on face to bounding-box alignment, and on other phenomena (face shapes, facial expressions, gender, hair and skin color, age, etc.) that are not relevant for the task at hand. The latent part of the regression output has the interesting mathematical feature of gathering information other than pose parameters and bounding-box parameters. Please see the revised paragraph \refcm{label-prob-1}.}
%	The latent part of the variable $\xvect$ is introduce to capture the variations in the observations that are not explained by the head pose (light variations is an example of the type of phenomena captured by the latent part of $\xvect$).

	\qa{Also,why the number of the parameters impacts the performance. What is the contribution of the low to high mapping? The impact of K on the performance ? how to choose K, and why the selected K is meaningful ?
Again, for the paper, performance is one key factor, but explaining the logic behind the performance is more meaningful. }
{In this paper we adopt a Gaussian mixture model, namely a parametric model. GMM models are extremely well understood from statistical and computational points of view. The number of model parameters is dictated by the number of parameters of a multivariate Gaussian distribution and by the number of Gaussian components ($K$), (which is discussed below). However, the number of parameters of an unconstrained GMM is quadratic in the dimension of the variable. Hence, the size of the training dataset required to reliably estimate a conventional GMM would become prohibitively high for the dimensions considered in the paper ($D=1888$). This is why an inverse regression strategy is adopted, making the number of parameters linear in the input variable dimension rather than quadratic. This drastically reduces the model size in practice, making it tractable. Please see the revised paragraph \refcm{inverse-def}.

The contribution of high-to-low mapping goes as follows: the high-dimensional space of face features embeds a low-dimensional nonlinear manifold. In our case the dimension of this manifold corresponds to the dimension of the output and is composed of an observed part and of a latent part. Therefore, one possible interpretation of the method is a unification of regression (fully observed output) and manifold learning (fully latent output). 

We agree that the selection of the number of Gaussian components, $K$, is important. In our model, the number of Gaussian components is equivalent to the number of affine transformations.
 As was already shown on Figure~\ref{fig:noiseDetection}, when K increases, the error decreases until it reaches a minimum. A large K implies more parameters to be learnt and also a higher risk to overfit the training dataset. The choice $K=50$ was validated experimentally using the means absolute error (MAE). We added another validation based on calculating an information-theoretic criterion, namely the Bayesian information criterion (BIC), that confirms our experimental choice. Please refer to \textbf{Figure~\ref{fig:bic}, Table \ref{table:BIC}} and to \refcm{label-exp-1}.
}
\end{answerreviewer2}

\end{coverletter}

\twocolumn
\setcounter{page}{1}



==> answers-tip.tex <==
Answers to questions:

The bios and photos are attached (they were already sent with the other files)

Financial section: The work of R. Horaud was PARTIALLY supported by ...

Emails:
vincent.drouard@inria.fr
radu.horaud@inria.fr
antoine.deleforge@inria.fr
sileye.ba@orah.co
george.evangelidis@gmail.com

The postal codes are correct

There is no page range for [37].


==> bios-tip.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photo-vincent_drouard.jpg}}]{Vincent Drouard}
received the M.Sc. in applied mathematics from the school of engineering, university of Nice Sophia-Antipolis in 2013. He is currently a Ph.D. student at the university of Grenoble Alpes (UGA) and member of the PERCEPTION team at INRIA Grenoble Rh\^one-Alpes. In 2015 he received the best student paper award (second place) at the IEEE International Conference on Image Processing.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photo-Radu-Horaud.jpg}}]{Radu Horaud} 
received the B.Sc. degree in Electrical Engineering, the M.Sc. degree
in Control Engineering, and the Ph.D. degree in Computer Science from
the Institut National Polytechnique de Grenoble, France. In 1982-1984 he was a post-doctoral fellow with the Artificial Intelligence Center, SRI International, Menlo Park, CA.
Currently he holds a position of director of research with INRIA Grenoble Rh\^one-Alpes, where
he is the founder and head of the PERCEPTION team. His
research interests include computer vision, machine learning, audio signal processing, 
audiovisual analysis, and robotics. Radu Horaud and his collaborators received numerous best paper awards. He is an area editor of the
\textit{Elsevier Computer Vision and Image Understanding}, a member of
the advisory board of the \textit{Sage International Journal of Robotics
  Research}, and an associate editor of the
\textit{Kluwer International Journal of Computer Vision}. 
He was program co-chair of IEEE ICCV'01 and of ACM ICMI'15.
In 2013 Radu Horaud was awarded an ERC Advanced Grant for his project \textit{Vision and Hearing in Action} (VHIA).
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,
height=1.25in,clip,keepaspectratio]{photo-antoine_deleforge.jpg}}]{Antoine Deleforge} is a tenured research scientist at INRIA with the PANAMA team, Rennes, France, since 2016. He received the B.En. (2008) and M.Sc. (2010) degrees in computer science and mathematics from ENSIMAG, Grenoble, France, and the M.Sc. (research track) degree in computer graphics, vision and robotics from the Universit\'e Joseph Fourier, Grenoble. In 2010-2013 he prepared a Ph.D in the PERCEPTION team, INRIA Grenoble Rh\^one-Alpes, and received the Ph.D. degree in computer science and applied mathematics in November 2013 from the university of Grenoble. In 2014-2015 he was a post-doctoral fellow in the audio group of the Multimedia Communications and Signal Processing chair of the Friedrich-Alexander university, Erlangen, Germany. His research interests are in machine learning, statistics and auditory scene analysis.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,
height=1.25in,clip,keepaspectratio]{photo-sileye_ba.png}}]{Sil\`{e}ye Ba}
received the M.Sc. (2000) in applied mathematics and signal processing from University of Dakar, Dakar, Senegal, and the M.Sc. (2002) in mathematics, computer vision, and machine learning from Ecole Normale Sup\'erieure de Cachan, Paris, France. From  
2003 to 2009 he was a PhD student and then a post-doctoral researcher at IDIAP Research Institute, Martigny, Switzerland,
where he worked on probabilistic models for object tracking and human activity recognition. From 2009 to 2013, he was a researcher at Telecom Bretagne, Brest, France working on variational models for multi-modal geophysical data processing. From 2013 to 2014 he worked at RN3D Innovation Lab, Marseille, France, as a research engineer, where he used computer vision and machine learning principles and methods to develop human-computer interaction software tools. From  2014 to 2016 he was a researcher in the PERCEPTION
team at INRIA Grenoble Rh\^one-Alpes, working on machine learning and computer vision models for human-robot interaction. Since May 2016 he is a computer vision scientist with VideoStitch, Paris.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in, height=1.25in,clip,keepaspectratio]{photo-georgios_evangelidis.jpg}}]{Georgios Evangelidis}
is a senior computer vision scientist at Daqri International. He received his Ph.D. in Computer Engineering from the University of Patras, Patras, Greece, in 2008. He joined  the Multimedia Pattern Recognition group at Fraunhofer IAIS, Bonn, Germany as a post-doctoral researcher (2009-2010) and the PERCEPTION
team at INRIA Grenoble Rh\^one-Alpes, France as a researcher (2012-2016). His expertise includes 3D geometry, depth sensors, action recognition and SLAM. 
\end{IEEEbiography}

